ATCO2 corpus: A Large-Scale Dataset for Research on Automatic Speech Recognition and Natural Language Understanding of Air Traffic Control Communications

Personal assistants, automatic speech recognizers and dialogue understanding systems are becoming more critical in our interconnected digital world. A clear example is air traffic control (ATC) communications. ATC aims at guiding aircraft and controlling the airspace in a safe and optimal manner. These voice-based dialogues are carried between an air traffic controller (ATCO) and pilots via very-high frequency radio channels. In order to incorporate these novel technologies into ATC (low-resource domain), large-scale annotated datasets are required to develop the data-driven AI systems. Two examples are automatic speech recognition (ASR) and natural language understanding (NLU). In this paper, we introduce the ATCO2 corpus, a dataset that aims at fostering research on the challenging ATC field, which has lagged behind due to lack of annotated data. The ATCO2 corpus covers 1) data collection and pre-processing, 2) pseudo-annotations of speech data, and 3) extraction of ATC-related named entities. The ATCO2 corpus is split into three subsets. 1) ATCO2-test-set corpus contains 4 hours of ATC speech with manual transcripts and a subset with gold annotations for named-entity recognition (callsign, command, value). 2) The ATCO2-PL-set corpus consists of 5281 hours of unlabeled ATC data enriched with automatic transcripts from an in-domain speech recognizer, contextual information, speaker turn information, signal-to-noise ratio estimate and English language detection score per sample. Both available for purchase through ELDA at http://catalog.elra.info/en-us/repository/browse/ELRA-S0484. 3) The ATCO2-test-set-1h corpus is a one-hour subset from the original test set corpus, that we are offering for free at https://www.atco2.org/data. We expect the ATCO2 corpus will foster research on robust ASR and NLU not only in the field of ATC communications but also in the general research community.

==> authors/default.tex <==


\author[$\star$,1,2]{Juan Zuluaga-Gomez}
\author[3]{Karel Vesel\'{y}}
\author[3,4]{Igor Szöke}
\author[1,3]{Petr Motlicek}
\author[3]{Martin Kocour}
\author[5]{Mickael Rigault}
\author[5]{Khalid Choukri}
\author[1,3]{Amrutha Prasad}
\author[1]{Seyyed Saeed Sarfjoo}
\author[1]{Iuliia Nigmatulina}
\author[6]{Claudia Cevenini}
\author[7]{Pavel Kol\v{c}árek}
\author[8]{Allan Tart}
\author[3]{Jan \v{C}ernocký}

\affil[1]{Idiap Research Institute, Martigny, Switzerland}
\affil[2]{Ecole Polytechnique Federale de Lausanne (EPFL), Lausanne, Switzerland}
\affil[3]{Brno University of Technology, Speech@FIT, IT4I CoE, Brno, Czech Republic}
\affil[4]{ReplayWell, Brno, Czech Republic}
\affil[5]{Evaluations and Language Resources Distribution Agency (ELDA), Paris, France}
\affil[6]{Honeywell, Brno, Czech Republic}
\affil[7]{Romagna Tech, Forli, Italy}
\affil[8]{OpenSky Network, Burgdorf, Switzerland} 
\affil[$^{~\star}$]{Corresponding author: \textbf{juan-pablo.zuluaga@idiap.ch}}

\keywords{Air Traffic Control Communications, Natural Language Processing, Automatic Speech Recognition}

==> chapters/e2e_asr.tex <==
\subsection{End-to-end ASR}

%\subsubsection{Prior Work}

End-to-end ASR aims at modeling AM + LM simultaneously and frequently employing character-based vocabularies, i.e., no human involvement to craft phonemes or tri-phones based lexicons. E2E systems are mostly fine-tuned with connectionist temporal classification (CTC) loss~\cite{graves2006connectionist}, which enables alignment-free training. Recently, E2E ASR yields state-of-the-art (SOTA) performance in many corpora. For instance, attention-based (e.g., Transformers) have become the \textit{de facto} choice for E2E acoustic modeling~\cite{baevski2020wav2vec,baevski2020effectiveness,babu2021xls}. A typical pipeline of and E2E model at inference time is depicted in Figure~\ref{fig:hb-vs-e2e-asr}.

Even though LMs are not needed in E2E systems, several prior work has demonstrated that integrating LMs by shallow fusion\footnote{For instance, combining LM and E2E ASR scores at inference time .} decrease WERs ~\cite{inaguma2019transfer,baevski2020effectiveness}. For example, one can train a n-gram LM based on Kneser–Ney smoothing~\cite{ney1994structuring} and then perform shallow. 

\subsubsection{Experimental Setup}

\quad \textbf{Wav2Vec 2.0}: we perform experiments with the well-known Wav2Vec 2.0~\cite{baevski2020wav2vec} (from now on w2v2). We fetch w2v2 pre-trained weights from HuggingFace platform~\cite{wolf-etal-2020-transformers}. Then, the model is fine-tuned on the ASR task with ATCO2 data. We provide a baseline experimentation with two different w2v2 checkpoints.
First, \mbox{i)~\textit{w2v2-B:}} BASE model with 95M parameters, pre-trained on train-set 960\,h LibriSpeech~\cite{panayotov_librispeech_ICASSP2015}. 
Second, \textit{w2v2-L-60K:} LARGE-960h-LV60K model with 317M parameters pre-trained on LibriSpeech + 60k\,h from LibriVox project i.e., Libri-Light~\cite{kahn2020libri} during and then fine-tuned on LibriSpeech. 
\vspace{0.2cm}

\textbf{Hyperparameters}: all experiments use the same set of hyperparameters. We fine-tune each model for 10k steps, with a 500-step warm-up phase ($\sim$10\% of total updates). Learning rate is increased linearly until $1e-4$ during warm-up, then it linearly decays. We fine-tune each model on an NVIDIA GeForce RTX 3090 with an effective batch size of 72 (batch size of 24, gradient accumulation of 3). We added a linear layer on top with dimension equal to the size of our character-based vocabulary\footnote{We keep simple our recipe by using characters as output of the network. Our vocabulary has a size of 32, accounting for all letters from English and some special symbols.}. We use CTC loss function~\cite{graves2006connectionist} and Adam optimizer~\cite{diederik2015adam} for fine-tuning each model. 
\vspace{0.2cm}

\textbf{Language model (LM):} we concatenate all text transcripts and train trigram LMs with KenLM\footnote{KenLM Python library in: \url{https://github.com/kpu/kenlm}.} toolkit to train a trigram LM. We then use PyCTCDecode library to fuse LM and w2v2 log probabilities\footnote{PyCTCDecode library in: \url{https://github.com/kensho-technologies/pyctcdecode}.} i.e., shallow fusion. We set $\alpha=0.5$ and $\beta=1.5$, which corresponds to the LM and length score normalization weights. We set the beam size to 100. 
\vspace{0.2cm}


\textbf{Data augmentation:} we apply a data augmentation strategy similar to~\cite{park2019specaugment}. We mask the input sequence with a probability $p=0.075$, and $M=12$ consecutive frames. We also use an activation and attention dropout of 0.05. These hyperparameters follow closely the original Wav2Vec 2.0 implementation~\cite{baevski2020wav2vec}.



==> chapters/metrics.tex <==

\subsection{Metrics} 
\label{subsec:metrics}

We list below the main performance metrics utilized in this paper. 

\subsubsection{Word error rate}

Word error rate (WER) is the most standard approach to evaluate the performance of an ASR system. This metric specifically compares an utterance's ground truth transcript against the hypothesized word sequence by the ASR system. The WER metric is fed with three different errors, i.e., the number of substitutions (S), insertions (I), and deletions (D), over the sum of all words in the transcript. In the case that there are N words in the reference transcript, we can calculate WER as follows:

\begin{equation}
    \label{eq:wer}
    WER=\frac{I + D + S}{N} \times 100.
\end{equation}

\subsubsection{F1-score}

In statistical analysis of binary classification, the F-score or F-measure is a measure of a test's accuracy. F1-\textit{score} is the harmonic mean of the precision and recall, as depicted in Equation~\ref{eq:f1-score}. Specifically, \textit{precision} is the number of true positive ($TP$) results divided by the number of all positive results (also includes those not identified correctly) i.e., $TP$ plus false positives ($FP$). \textit{Recall} is the number of $TP$ divided by the number of all samples that should have been identified as positive, i.e., $TP$ plus false negatives ($FN$). Precision and recall are depicted in the Equation~\ref{eq:precision} and~\ref{eq:recall}, respectively.

\begin{equation}
    \label{eq:precision}
    Precision = \frac{TP}{TP+FP}.
\end{equation}

\begin{equation}
    \label{eq:recall}
    Recall = \frac{TP}{TP+FN}.
\end{equation}

\begin{equation}
    \label{eq:f1-score}
    F1 = \frac{2*Precision*Recall}{Precision+Recall} = \frac{2*TP}{2*TP+FP+FN}.
\end{equation}


==> chapters/quality_estimation.tex <==
% Quality estimation for annotation.
\subsection{Quality Estimation of Audio Data}

\begin{figure}[t]
    % \widefigure
    \centering
    % \includegraphics[width=0.9\linewidth]{figures/data_flow.png}
    \includegraphics[width=0.9\linewidth]{figures/data_cleaning.pdf}
    \caption{Breakdown of data flow yield from raw data (recordings from data feeders) to the human annotated transcripts throughout the pipeline. This is a one-day snapshot from 9.2.2022.}
    \label{fig:data_flow}
\end{figure}

Alongside ATCO2 project, we integrated up to seven different metrics with the aim of assessing the quality of each sample present in the \textit{ATCO2 corpora}. For instance, we use the Equation~\ref{eq:quality-audio} to measure, rank and select the samples with the highest quality. Later, these were passed to the annotators for generating the ground truth transcripts and tags that are part of the \textit{ATCO2 test set corpus}.


\begin{equation}
    \label{eq:quality-audio}
    \begin{split}
        Score = \log(avg_{SNR} + e) + \log(num_{spk} + e) + \log\left(\dfrac{speech_{len}}{audio_{len}} + e\right) + LID_{score} \times 3~+ avg_{WordConf} \times 3 + \log(wrd_{cnt} + e),
    \end{split}
\end{equation}

where,

\begin{itemize}
    \item $avg_{SNR}$ — provides average SNR of speech in range <0, 40>. We want SNR to be as high as possible,
    \item $num_{spk}$ — provides the number of speakers in the audio in range of <1, 10>. More speakers detected in audio, the better,
    \item $speech_{len}$ — provides the amount of speech in seconds,
    \item $audio_{len}$ — provides the overall audio length. More speech detected in audio is better,
    \item $LID_{score}$ provides “probability” of audio being English in the range <0.00,1.00>, the higher, the better,
    \item $avg_{WordConf}$ - provides average confidence of the speech recognizer <0.00, 1.00>. We want data where the recognizer is confident. Higher is better,
    \item $wrd_{cnt}$ - provides the amount of words spoken in the range of <0, ~150>. The more words, the better.
\end{itemize}

The quality estimation from Equation~\ref{eq:quality-audio} was used to select the files with the highest quality for gold annotations. A breakdown of the pipeline is in Figure~\ref{fig:data_flow}, where only 0.6\,hrs of data are selected for gold annotations from 26\,hr-pool of audio data. We believe this is a robust quality scoring method because it gathers information from different systems, e.g., ASR, SNR and LID estimation. 
